Parametrization and Estimation of High-Rank Line-of-Sight MIMO Channels with Reflected Paths

High-rank line-of-sight (LOS) MIMO systems have attracted considerable attention for millimeter wave and THz communications. The small wavelengths in these frequencies enable spatial multiplexing with massive data rates at long distances. Such systems are also being considered for multi-path non-LOS (NLOS) environments. In these scenarios, standard channel models based on plane waves cannot capture the curvature of each wave front necessary to model spatial multiplexing. This work presents a novel and simple multi-path wireless channel parametrization where each path is replaced by a LOS path with a reflected image source. The model fully is valid for all paths with specular planar reflections and captures the spherical nature of each wave front. Importantly, it is shown that the model uses only two additional parameters relative to the standard plane wave model. Moreover, the parameters can be easily captured in standard ray tracing. The accuracy of the approach is demonstrated on detailed ray tracing simulations at 28 GHz and 140 GHz in a dense urban area.

==> extra.tex <==

%We assume that between 
% any pair For example, 
% while most
% commercial ray tracers, such as Remcomm's Wireless Insite
% \cite{Remcom} that we use in the simulations below,
% provide the path route for each multi-path component,
% the path route is not known when using measurement
% data.  Measurements generally only provide
% the angles of arrival $(\theta^r,\phi^r)$,
% the angles of departure $(\theta^t,\phi^t)$,
% and  the magnitude of the path gain  $g$.
% In synchronized systems, the absolute delay, $\tau$, 
% of the path may also be measured.
% However, the full path \eqref{eq:path_sequence}
% with the locations of the reflections is generally
% not directly measured.  Hence, we cannot apply
% the route tracing method above to estimate
% the RM model parameters.

% However, in this case, we show that the remaining parameters
% of the RM model can be found from a small number of
% additional measurements displaced from the reference
% TX and RX locations.  When the RM model
% parameters are learned via this method,
% we will call the learned the \emph{reflection model via displaced pairs (RM-DP)}.

\section{Validation}
As shown in Fig.~\ref{fig:remcom_beijing}, We use a partial area of Beijing city as the validation ray-tracing environment.
The environment consists of typical metropolitan office building structures, urban vegetation, and a relatively flat urban terrain.
To validate the model, we conduct the following experiment on this partial area of Beijing:
\begin{itemize}
    \item Take a large number, $N$, TX-RX to be the reference locations. As shown in  Fig.~\ref{fig:remcom_beijing}, $N=43$, red dots are the transmitters, and green dots are the receivers. Thus, there are 43 unique links. Let $\nbx^r_i$ and $\nbx^t_i$
    be the TX and RX locations for link $i$.
    \item Take a displacement of each TX and RX:  $\nby^r_i$ and $\nby^t_i$ where 
    $\|\nbx^r_i-\nby^r_i\|=d$ and $\|\nbx^t_i-\nby^t_i\|=d$ for some displacement distance $d$. Each time we displace on one of the multiple values of $d$, which are $\lambda$, $2\lambda$, $5\lambda$, $10\lambda$, $50\lambda$, and $100\lambda$ in our validation. As shown in Fig.~\ref{fig:move_direction}, the red point represents the reference location, \textcolor{red}{(to be added):}.
    \item Run ray tracing from each link $(\nbx^r_i,\nbx^t_i)$ to find all the paths.  Compute the complex channel gain
    $h_i$ from $\nbx^t_i$ to $\nbx^r_i$.
    \item Run ray tracing from each link $(\nby^r_i,\nby^t_i)$ to find all the paths.
    Compute the complex channel gain $\tilde{h}_i$ from $\nby^t_i$ to $\nby^r_i$. 
    \item From the ray tracing in step 3, we can make a prediction of the complex channel gain $\tilde{h}_i$ at the displaced point.
    Call this prediction $\widehat{h}_i$.  Compute the error using the PWA model, $\epsilon_i^{\rm PWA}$./
    \item We also fit the parameters of the reflected model for all the reflected paths.  (somehow)
    \item Then, we use the reflected model to compute the phases of all the paths at the displaced point and then make an estimate of
    the channel.  Compute the error using the RM model, $\epsilon_i^{\rm RM}$.
    \item In both cases, there will be some errors.
    \item Plot the average error for both models as a function of the displacement distance $d$.
\end{itemize}

\section{Updates Nov 30}
\textcolor{red}{(What we done):}
\begin{itemize}
    \item 1 reference TX-RX; 6 displaced TX-RX (1, 2, 5, 10, 50, 100 * $\lambda$ distance); Each has 39 unique Tx-Rx channels.
    \item Matching the reference TX-RX channels with \textbf{one of the six} displaced TX-RX channels (we call this one of six channel as Gamma Channel)
    \item path matching method: 
    \item path\_id = argmin(angles difference)
    \item add a restriction: |argmin(angles difference) - argmin(delay difference)|  $\leq$ 1 or 2
    \item Compute $\gamma$ angles for every matched path
    \item Then use \textbf{\textcolor{red}{another} one of the six displaced TX-RX} (we call this one of six channels as Validation Channel) to evaluate if the $\gamma$ angles can reduce the distance error (we call it as reflection model [RM] error).
    \item Also compute the \textbf{PWA} distance error.
    \item Compare \textbf{PWA} and \textbf{RM} estimated distance error.
\end{itemize}


\textcolor{red}{(What we found):}
\begin{enumerate}
    \item \textit{Remcom} ray-tracing angles result has tiny errors even in LOS paths
    \item \textit{Remcom} using light speed $= 2.996955055081703e8$ which is computed by LOS paths
    \item \textit{Remcom} phase result are not directly computed from the distance in NLOS paths, and we don't know how it is been calculated.
    \item \textit{Small} displacement-distance TX-RX can match more (around 20\% to 40\%) paths with the reference TX-RX than \textit{large} displacement-distance TX-RX.
    \item Unlike ideal LOS and one-reflection path we generated by math, because \textit{Remcom} has errors in angles, we can solve $\gamma$ values from \textbf{both} $s=1$ and $s=-1$ and do not need to consider the number of reflections
    \item There are some root solving methods can be used to compute the $\gamma$ angles from matched path pairs, and different methods we used and different "initial root guesses" we set in the functions may lead to different $\gamma$ results.
    \item We use \textit{scipy.optimize.root$\_$scalar} and "initial root guesses" $= 0$, $\pi$ to achieve following results. 
    Other functions may also works.

    \item Most of the cases $\gamma$ values are in $[-\pi$, $\pi]$.
    \item Most of the cases \textbf{RM} distance error is smaller than the \textbf{PWA}.
    \item When the distance between the Gamma Channel and the Validation Channel increases, the RM distance error increases.
    \item Because small displacement-distance Gamma channel can matched more paths with the reference channel, the overall error will smaller than using large displacement-distance Gamma channel.

\end{enumerate}

\textcolor{red}{(What we are considering):}
\begin{itemize}
    \item The \textbf{Phase problem} in ray tracing result, which make us cannot directly use the distance to compute the phase and then get the channel gain.
    \item We only compute the error of distance, but not error of complex channel gain here. 
    \item Better \textbf{path match method}
    \item For now, tx and rx displaced in the same direction, maybe we can try not in the same direction
\end{itemize}


\subsection{Update 12/1/2021}

Sundeep's suggestions:
\begin{itemize}
    \item Use the reference channel and the \textbf{smallest} displacement channel to estimate the parameters for all paths at the reference.  So if there $L$ paths, you will have $L$ parameter vectors \eqref{eq:param_high} for $\ell = 1,\ldots,L$.
    
    \item We now validate the model at other displacements
    (potentially larger than the ones we measured the parameters).
    
    \item At each validation displacement, compute the displacements $\nbx^r-\nbx^r_0$ and $\nbx^t-\nbx^t_0$.

    \item From \eqref{eq:dnlos} and the parameters \eqref{eq:param_high}, compute the predicted 
    channel gain from \eqref{eq:Hmn}
    \begin{equation}
        \widehat{H}(f) = \sum_{\ell=1}^L g_\ell \exp\left(
        2\pi i \left(\frac{fd_\ell(\nbx^r,\nbx^t)}{c} - f_c\tau_\ell\right)
        \right),
    \end{equation}
    where $g_\ell$ and $\tau_\ell$ are, respectively,
    the complex channel gain and delay at the reference
    location and carrier frequency $f_c$.
    
    \item Also compute the true channel gain 
    using the paths from the ray tracer:
    \begin{equation}
        H(f) = \sum_{\ell=1}^{L'} g_\ell' e^{2\pi i (f-f_c)\tau'_\ell},
    \end{equation}
    where $L'$ is the number of paths seen by the ray tracer,
    $g_\ell'$ includes the gain and phase,
    and $\tau_\ell'$ is the delay of the path.
    

    
\end{itemize}

\section{Things to Do}

\begin{itemize}
    \item Discuss how to get the parameters from ray tracing.
    \item Add the polarization.
    \item Add the discussion on the antenna elements.
    \item Add some simulations.
\end{itemize}

\section{Extra}
We use the following.  From \eqref{eq:dnlos}, we have that
\begin{align}
    \MoveEqLeft d(\nbx^r,\nbx^t)^2 = \|a + b + c\|^2 = \|a\|^2 + \|b\|^2 + \|c\|^2 \nonumber \\
    & + 2a^\intercal b + 2a^\intercal c + 
    2b^\intercal c,
\end{align}
where 
\begin{align}
    a &:=  c\tau\nbe_x \\
    b &:= \nbR_y(\theta^r)\nbR_z(-\phi^r)(\nbx^r_0-\nbx^r) \\
    c&:= \nbQ_z(s)\nbR_x(\gamma^t)
       \nbR_y(\theta^t)\nbR_z(-\phi^t)(\nbx^t_0-\nbx^t).
\end{align}
Hence we have 
\begin{align}
    \|a\|^2 &= (c\tau)^2 \|\nbe_x\|^2 = (c\tau)^2, \\
    \|b\|^2 &= b^\intercal b  \nonumber \\
    &= (\nbx^r_0-\nbx^r)^\intercal\nbR_z(-\phi^r)^\intercal \nonumber\\
    & \times \nbR_y(\theta^r)^\intercal\nbR_y(\theta^r)\nbR_z(-\phi^r)(\nbx^r_0-\nbx^r) \nonumber \\
    &= (\nbx^r_0-\nbx^r)^\intercal(\nbx^r_0-\nbx^r)  
    = \|\nbx^r_0-\nbx^r\|^2.
\end{align}

A benefit of the image model in Theorem~\ref{thm:high_order} is that the
parameters can be easily extracted from ray tracing.  First, taking a linearlization 
\begin{align} \label{eq:dsqexp}
    \MoveEqLeft d(\nbx^r,\nbx^t)^2 = (c\tau)^2 + 2c\tau (\nbu^r)^\intercal (\nbx^r_0-\nbx^r) \nonumber \\
         &+ 2c\tau (\nbu^t)^\intercal (\nbx^t_0)-\nbx^t) 
         + B
\end{align}

\subsection{Checking that the formula is correct in LOS case}
For the LOS case, $\gamma = 0\degree$ and $s=-1$, the following equation holds:
\begin{align}
    \MoveEqLeft 
        d(\nbx^r,\nbx^t) = \Bigl\| 
        c\tau\nbe_x +  \nbR_y(\theta^r)\nbR_z(-\phi^r)(\nbx^r_0-\nbx^r)
        \nonumber \\
       & + \nbQ_z(-1)\nbR_x(0\degree)
       \nbR_y(\theta^t)\nbR_z(-\phi^t)(\nbx^t_0-\nbx^t) 
    \Bigr\|,
    \label{eq:dlos}
\end{align}
where we calcuate the AoA by $cart2sph(\nbx^t_0 - \nbx^r_0)$, and AoD by $cart2sph(\nbx^r_0 - \nbx^t_0)$.

And we will have:
\[
    \theta^r = -\theta^t;
\]
\[
    |\phi^r-\phi^t| = \pi.
\]
Then,
\begin{align*}
\nbu^r &= (\cos(\phi^r)\cos(\theta^r), 
    \sin(\phi^r)\cos(\theta^r), \sin(\theta^r)) \\
    &= (\cos(\phi^r)\cos(-\theta^t), 
    \sin(\phi^r)\cos(-\theta^t), \sin(-\theta^t)) \\
    &= (\cos(\phi^r)\cos(\theta^t), 
    \sin(\phi^r)\cos(\theta^t), -\sin(\theta^t))\\
    &= (-\cos(\phi^t)\cos(\theta^t), 
    -\sin(\phi^t)\cos(\theta^t), -\sin(\theta^t))\\
    &= -(\cos(\phi^r)\cos(\theta^t), 
    \sin(\phi^r)\cos(\theta^t), \sin(\theta^t)) \\
    &=  -\nbu^t,
\end{align*}
proof the $\nbu^r = - \nbu^t$ when LOS cases.

% For the LOS case, we know
% \[
%     \nbu^r = - \nbu^t.
% \]
% This corresponds to $\theta^r = -\theta^t$, $s=-1$ and $|\phi^r-\phi^t| = \pi$

% \[
%     \nbu^t = \nbQ_z(-1)\nbu^r.
% \]

where
\begin{subequations}
\begin{align}
    \nbu^r &:= (\nbR_y(\theta^r)\nbR_z(-\phi^r))^T \nbe_x \\
    \nbu^t &:= (\nbR_y(\theta^t)\nbR_z(-\phi^t))^T \nbe_x,
\end{align}
\end{subequations}
and $B$ are the quadratic
terms in the displacements $\nbx^r-\nbx^r_0$
and $\nbx^t-\nbx^t_0$.
Using the expressions for the rotation matrices
\eqref{eq:rotmatrix} we get that $\nbu^r$
and $\nbu^t$ is of the form \eqref{eq:usph}.
Since the ray tracing provides these
angles, we obtain $\theta^r$, $\theta^t$, 
$\phi^r$, $\phi^t$. 

Hence, we only need to extract $s$ and 
$\gamma$. For this purpose, 
let's consider the quadratic terms, 
$B$ in \eqref{eq:dsqexp}.  These terms are
\begin{align}
    B &:= \|\nbx^t-\nbx^t_0\|^2 + 
    \|\nbx^r-\nbx^r_0\|^2  \nonumber \\
    &+ 2(\nbv^r)^\intercal \nbQ_z(s) R_x(\gamma^t)
    \nbv^t,
\end{align}
where
\begin{subequations}
\begin{align}
    \nbv^r &:= \nbR_y(-\theta^r)\nbR_z(\phi^r)(\nbx^r_0-\nbx^r), \\
    \nbv^t &:= \nbR_y(-\theta^t)\nbR_z(\phi^t)(\nbx^t_0-\nbx^t).
\end{align}
\end{subequations}

\begin{figure*}[t]
\footnotesize
\centering
\includegraphics[width=0.9 \linewidth]{Figures/ecdf_plot_lambda_fix.png}
\caption{ecdf plot for fixed direction at different distance}
\label{fig:ecdf_lambda_fix}
\vspace{-2mm}
\end{figure*}

\begin{figure} 
  \centering
  \includegraphics[width=1 \linewidth]{Figures/ecdf_plot_model_fix.png}
  \caption{ecdf plot for fixed direction of different models}
  \label{fig:ecdf_model_fix}
\end{figure}

\begin{figure*}[t]
\footnotesize
\centering
\includegraphics[width=0.9 \linewidth]{Figures/ecdf_plot_lambda_rnd.png}
\caption{ecdf plot for randomized direction at different distance}
\label{fig:ecdf_lambda_rnd}
\vspace{-2mm}
\end{figure*}

\begin{figure} 
  \centering
  \includegraphics[width=1 \linewidth]{Figures/ecdf_plot_model_rnd.png}
  \caption{ecdf plot for randomized direction of different models}
  \label{fig:ecdf_model_rnd}
\end{figure}

\begin{figure} 
  \centering
  \includegraphics[width=1 \linewidth]{Figures/move_direction_v2.png}
  \caption{Another option for Fig.~\ref{fig:move_direction}.}
  \label{fig:move_direction_v2}
\end{figure}



A second method is to run ray tracing once at the array centers
and extract the PWA parameters.  The MIMO channel matrix can then be
estimated for arbitrary arrays geometries and orientations.   

% We place TX and RX arrays in the Beijing area used in the previous sections in one of three test locations: Test (a), (b) and (c).
% The 2D (top view) of the 
% For the purpose of testing the reflection model ability on the wide aperture MIMO system in both LOS and NLOS environments, we create three test cases (a), (b), and (c).
% In the Test (a), all links in TX and RX array are in a LOS link state.
% For the Test (b) and (c), we insert a obstacle of size 2m $\times$ 3m $\times$ 4m to block the rays, and in which case, all the links are in a NLOS case.
% In Test (b), the obstacle is oriented in the X-axis (east-west), while in Test (c), it is oriented in the Y-axis.

On each of the three settings, we follow the same procedure.
As illustrated in Fig.~\ref{fig:TXRot},
our first step is to fix the orientation of the RX array, which is aligned on the boresight and faces the center of the TX array.
And for each $\phi \in [-180^{\circ},180^{\circ}]$ with $15^{\circ}$ steps, we create a TX array pointing at an angle $\phi$.
At each TX rotation step, we run ray tracing between all the TX-RX element pairs to obtain the true channel $\nbH(\phi)$ at frequency \SI{140}{GHz}, where each one element out of 4096 (64 $\times$ 64) can be derived from \eqref{eq:Hmn}.
The channel matrix $\nbH$ is represented by:
\begin{equation} \label{eq:H4096}
    \nbH = \begin{bmatrix} 
    H_{11} & \dots  & H_{1N_{\rm rx}}\\
    \vdots & \ddots & \vdots\\
    H_{N_{\rm tx}1} & \dots  & H_{N_{\rm tx}N_{\rm rx}} 
    \end{bmatrix},
\end{equation}
where $N_{\rm tx} = 64$ is the number of elements of TX array, $N_{\rm rx} = 64$ is the number of elements of RX array, and each element of $\nbH$ is defined by \eqref{eq:Hmn}.


In order to estimate the channel by reflection model, we select the centroids of the TX and RX arrays as the reference pair, select two displaced pairs randomly, and run ray tracing on each pair separately.
Then, we can estimate the $\gamma$, $s$ if choose to use \eqref{eq:dnlos}, or compute $\nbU$, $\nbg$ if choose to use \eqref{eq:dnlosUg}, bearing in mind that displaced pairs are not required for \eqref{eq:dnlosUg}, and finally compute the estimated channel $\widehat{\nbH}(\phi)$.
In our case, we estimate the parameters using the RM-DP method.
We also compute the estimated channel by PWA model from the distance formula \eqref{eq:dpwa}.

With the channel matrix $\nbH$, we use the singular value decomposition (SVD) to find the singular vector $\nbs$.
Then the MIMO channel capacity is defined as:
\begin{equation}
R=\sum_{i=1}^{r} \log_2 \left(1+\gamma_{i} x_{i}\right)
\end{equation}
where $r$ represents the number of virtual streams to be used, and
\begin{equation}
\gamma_{i}=\frac{s_{i}^{2} E_{x}}{N_{0}}
\end{equation}
is SNR on virtual stream $i$ if all power is allocated to stream, $x_i$ is the fraction of power allocated to the virtual stream $i$.
The $s_i$ represents the $i$-th singular value in the singular vector $\nbs$ 
We also take $E_{x}=\SI{23}{dBm}$ in linear scale,
and the $N_0$ is defined as following:
\begin{align}
N_0 &= K_t+10log_{10}(B)+N_f\nonumber,
\end{align}
in linear scale,
where the Johnson–Nyquist noise $K_t$ sets to \SI{-174}{dBm}, the bandwidth $B$ is \SI{2}{GHz}, and the noise figure $N_f$ equals to \SI{3}{dB}.

We implement the optimal rank selection as the power allocation strategy, which means that we uniformly allocate the transmit power to top $r$ virtual stream. 
In this case, the fraction of power allocated $x_i$ is defined as:
\begin{align}
    x_i &= \frac{1}{r}\nonumber,
\end{align}
and the value of r is determined by maximising the capacity of $R$:
\begin{align}
    r &= \argmaxtopdown_{r \in [1, \rank(\nbH)]} R \nonumber,
\end{align}

In each of the three tests we have described above, we estimate the MIMO channel $\widehat{\nbH}$ using the reflection model, the PWA model, and the constant model, and then measure the maximum channel capacity $R$. 
In the first and second rows of Fig.~\ref{fig:capacity}, top-down and 3D views are shown to illustrate the three different simulation environments.
It is worth noting that the location of TX and RX for all three test cases are the same.
Moreover, the orientation of the added obstacle in Test (b) and (c) is variant in order to simulate the different situations in which the rays are blocked.


A second method is to run ray tracing once at the array centers
and extract the PWA parameters.  The MIMO channel matrix can then be
estimated for arbitrary arrays geometries and orientations.   

% We place TX and RX arrays in the Beijing area used in the previous sections in one of three test locations: Test (a), (b) and (c).
% The 2D (top view) of the 
% For the purpose of testing the reflection model ability on the wide aperture MIMO system in both LOS and NLOS environments, we create three test cases (a), (b), and (c).
% In the Test (a), all links in TX and RX array are in a LOS link state.
% For the Test (b) and (c), we insert a obstacle of size 2m $\times$ 3m $\times$ 4m to block the rays, and in which case, all the links are in a NLOS case.
% In Test (b), the obstacle is oriented in the X-axis (east-west), while in Test (c), it is oriented in the Y-axis.

On each of the three settings, we follow the same procedure.
As illustrated in Fig.~\ref{fig:TXRot},
our first step is to fix the orientation of the RX array, which is aligned on the boresight and faces the center of the TX array.
And for each $\phi \in [-180^{\circ},180^{\circ}]$ with $15^{\circ}$ steps, we create a TX array pointing at an angle $\phi$.
At each TX rotation step, we run ray tracing between all the TX-RX element pairs to obtain the true channel $\nbH(\phi)$ at frequency \SI{140}{GHz}, where each one element out of 4096 (64 $\times$ 64) can be derived from \eqref{eq:Hmn}.
The channel matrix $\nbH$ is represented by:
\begin{equation} \label{eq:H4096}
    \nbH = \begin{bmatrix} 
    H_{11} & \dots  & H_{1N_{\rm rx}}\\
    \vdots & \ddots & \vdots\\
    H_{N_{\rm tx}1} & \dots  & H_{N_{\rm tx}N_{\rm rx}} 
    \end{bmatrix},
\end{equation}
where $N_{\rm tx} = 64$ is the number of elements of TX array, $N_{\rm rx} = 64$ is the number of elements of RX array, and each element of $\nbH$ is defined by \eqref{eq:Hmn}.


In order to estimate the channel by reflection model, we select the centroids of the TX and RX arrays as the reference pair, select two displaced pairs randomly, and run ray tracing on each pair separately.
Then, we can estimate the $\gamma$, $s$ if choose to use \eqref{eq:dnlos}, or compute $\nbU$, $\nbg$ if choose to use \eqref{eq:dnlosUg}, bearing in mind that displaced pairs are not required for \eqref{eq:dnlosUg}, and finally compute the estimated channel $\widehat{\nbH}(\phi)$.
In our case, we estimate the parameters using the RM-DP method.
We also compute the estimated channel by PWA model from the distance formula \eqref{eq:dpwa}.

With the channel matrix $\nbH$, we use the singular value decomposition (SVD) to find the singular vector $\nbs$.
Then the MIMO channel capacity is defined as:
\begin{equation}
R=\sum_{i=1}^{r} \log_2 \left(1+\gamma_{i} x_{i}\right)
\end{equation}
where $r$ represents the number of virtual streams to be used, and
\begin{equation}
\gamma_{i}=\frac{s_{i}^{2} E_{x}}{N_{0}}
\end{equation}
is SNR on virtual stream $i$ if all power is allocated to stream, $x_i$ is the fraction of power allocated to the virtual stream $i$.
The $s_i$ represents the $i$-th singular value in the singular vector $\nbs$ 
We also take $E_{x}=\SI{23}{dBm}$ in linear scale,
and the $N_0$ is defined as follows:
\begin{align}
N_0 &= K_t+10log_{10}(B)+N_f\nonumber,
\end{align}
in linear scale,
where the Johnson–Nyquist noise $K_t$ sets to \SI{-174}{dBm}, the bandwidth $B$ is \SI{2}{GHz}, and the noise figure $N_f$ equals to \SI{3}{dB}.

We implement the optimal rank selection as the power allocation strategy, which means that we uniformly allocate the transmit power to top $r$ virtual stream. 
In this case, the fraction of power allocated $x_i$ is defined as:
\begin{align}
    x_i &= \frac{1}{r}\nonumber,
\end{align}
and the value of r is determined by maximizing the capacity of $R$:
\begin{align}
    r &= \argmaxtopdown_{r \in [1, \rank(\nbH)]} R \nonumber,
\end{align}

In each of the three tests we have described above, we estimate the MIMO channel $\widehat{\nbH}$ using the reflection model, the PWA model, and the constant model, and then measure the maximum channel capacity $R$. 
In the first and second rows of Fig.~\ref{fig:capacity}, top-down and 3D views are shown to illustrate the three different simulation environments.
It is worth noting that the location of TX and RX for all three test cases are the same.
Moreover, the orientation of the added obstacle in Test (b) and (c) is variant in order to simulate the different situations in which the rays are blocked and 
